ZebraLancer: Decentralized Crowdsourcing of Human Knowledge atop Open Blockchain

We design and implement the first private and anonymous decentralized crowdsourcing system ZebraLancer, and overcome two fundamental challenges of decentralizing crowdsourcing, i.e., data leakage and identity breach. First, our outsource-then-prove methodology resolves the tension between the blockchain transparency and the data confidentiality to guarantee the basic utilities/fairness requirements of data crowdsourcing, thus ensuring: (i) a requester will not pay more than what data deserve, according to a policy announced when her task is published via the blockchain; (ii) each worker indeed gets a payment based on the policy, if he submits data to the blockchain; (iii) the above properties are realized not only without a central arbiter, but also without leaking the data to the open blockchain. Second, the transparency of blockchain allows one to infer private information about workers and requesters through their participation history. Simply enabling anonymity is seemingly attempting but will allow malicious workers to submit multiple times to reap rewards. ZebraLancer also overcomes this problem by allowing anonymous requests/submissions without sacrificing accountability. The idea behind is a subtle linkability: if a worker submits twice to a task, anyone can link the submissions, or else he stays anonymous and unlinkable across tasks. To realize this delicate linkability, we put forward a novel cryptographic concept, i.e., the common-prefix-linkable anonymous authentication. We remark the new anonymous authentication scheme might be of independent interest. Finally, we implement our protocol for a common image annotation task and deploy it in a test net of Ethereum. The experiment results show the applicability of our protocol atop the existing real-world blockchain.

==> anonymous.tex <==
%!TEX root = main.tex


%\section{Privacy Preserving Decentralized Crowdsourcing System: Supporting Worker Anonymity}\label{sec5}
\section{Further Step Towards Anonymity}\label{sec5}

Our basic protocol in previous section enables us to facilitate decentralized crowdsourcing without breaching the privacy of answers. However, it is easy to see that the anonymity of either workers or requesters is not protected. For example, suppose worker $W_i$ participates in multiple tasks, then everyone can link those tasks from his public key and certificate. If the tasks are carefully crafted, one may even infer the real identity of the worker \cite{YZR15}. In this section, we upgrade our basic protocol to further support the anonymity and tackle {\em Challenge 2}.

\ignore{%%%%%%
\begin{table}[!h]
\centering
\caption{Key notations used in our anonymous credential scheme.}
\begin{tabular}{l|l}
\hline
Notation            & Definition            \\ \hline
$C$  & Blockchain address of a contract        \\
$SK_{CA}$,$PK_{CA}$  & SK and PK of CA   \\
$SK_W$,$PK_W$  & SK and PK of a worker   \\
$cert:=(W,PK_W,\delta)$           & Certificate        \\
%$cert:=(PK,\delta)$           & Anonymous certificate        \\
$\delta:=sign(cert,SK_{CA})$   & Signature of CA         \\
$vrfy(cert,\delta,PK_{CA})$ & Signature verification function\\
$h(\cdot)$    &collision-resistant hash function         \\
$token := h(PK\|addr)$       &anonymous token \\\hline
\end{tabular}
\end{table}
}%%%%%%%

%\noindent \textbf{Overview} A trivial way of using PKI to prevent Sybil attack is to enforce workers submit answers along with their certificates, but ones can explore the privacy of workers by linking tasks to their certificates. Facing the challenging privacy issue in data crowdsourcing, we invite this scheme to maximize the privacy of workers by minimizing linkability.
%The scheme is based on and compatible with the previous PKI scheme. The idea behind the scheme is that a worker shows an anonymous credential including an anonymous token and a NIZK proof. The token is uniquely generated from the digital certificate and the address of a contract, and the proof $\pi$ can convince the contract that: 1. the worker knows a valid certificate signed by CA; 2. and, the worker owns the certificate because she knows the secret key paired to the public key in the certificate. Recall the privacy requirements P1 and P2 discussed in Section II. The scheme can realize both of them, and meanwhile allows a contract to identify workers.

\smallskip
\noindent{\bf Intuition}. The new threat in the anonymous setting is that a malicious worker may submit more than one answer. As shown in Fig.\ref{anonymous}, we examine our requirements more carefully as: revealing whether a worker submits twice, but neither linking the worker to his any answer nor linking any two tasks joined by him. We put forth a new cryptographic tool called {\em \sameprefix-linkable} anonymous credential. In the scheme, a token is generated from the address of the task contract that the worker is joining, his certificate, and some metadata by a hash function $H(\cdot)$. Such a token generally reveals nothing about the real certificate of a worker, as well as has a delicate linkability: when two tokens are generated from a same contract address and a same certificate, everyone can tell that they are from the same worker. In this way, we can have an anonymous system with keeping workers accountable.

To approach the above scheme, we again leverage the tool of zk-SNARK. The worker $W_i$ simply hashes $\alpha_\huaC, PK_i, cert_i$, and $H(SK_i)$ to obtains a token $t_i$. He then attests a proof $\pi_i$ that $t_i$ is computed correctly. When we model the hash function $H(\cdot)$ as a random oracle, it leaks nothing about its inputs; moreover, $\pi_i$ is generated in a {\em zero-knowledge} way. Thus the link between the worker identity and the submitted data can be broken. If a worker $W_i$ generates two tokens in two different contracts, respectively, the hash function and the zero-knowledge property still ensure that no one can tell they are actually committing to the same certificate. Also, it is straightforward that if a worker submits twice to one contract, everybody notices it, because two tokens will be unrelated. %identical.
%
%We remark that our current construction of the \sameprefix-linkable anonymous credential relies on the random oracle assumption and zk-SNARK, it is worthy of a systematic study to remove those assumptions, and we leave it as an open problem.
%Such an anonymous credential in general is unlinkable, while at the same time, it has a delicate linkability that only when




\begin{figure}[!h]
%\vspace{-4.5mm}
\centering
\includegraphics[width=4.5cm]{fig6.eps}
\caption{Flows of anonymous answer submission.}
\label{anonymous}
%\vspace{-2.5mm}
\end{figure}



\smallskip
\noindent \textbf{Anonymous protocol.}  The below is our anonymous protocol on top of blockchain. Many of the steps are similar to the basic protocol, here we mainly list the difference.  %As illustrated in Fig.4, the scheme has the following five algorithms:
\begin{itemize}
\item {\em Round 0}. Same as basic protocol.

\item {\em Round 1}. Almost the same as before, the requester complies and sends a contract to the blockchain. The only two exceptions are: (i) the smart contract can identify workers by checking their anonymous credentials (scheme details shown in the next round), so that participating workers will not reveal either their signatures or certificates; (ii) the requester also shows an anonymous credential instead of her signature and certificate to the contract $\huaC$, to attest her valid identity. See Alg.\ref{contract:anonymous} for the different part.

\item {\em Round 2}. The worker $W_i$ prepares a {\em one-time} blockchain account $\alpha_i$ to interact with the blockchain (i.e. to send his answer and receive the reward),\footnote{One-time account can prevent an adversary exploring a worker's participation history through looking for this account. We remark that our anonymous protocol is only focusing on the application layer such as the crowdsourcing functionality that is built on top of the blockchain infrastructure. If the underlying blockchain layer supports anonymous transaction, the worker can re-use his account $\alpha_i$. We further remark that the worry of the privacy leakage through Internet infrastructure is out the scope of this paper, and workers can use the best state-of-the-art technology such as the use of Tor in Zcash.}
and then submits $(t_i,\pi_i,C_i,\alpha_i)$, where $t_i=H(\alpha_\huaC,PK_i,cert_i,H(SK_i))$, and $H(\cdot)$ is a variable-input-length hash function that is modeled as a random oracle.
    $\pi_i$ is proving that $t_i$ and some common knowledge, including $\alpha_\huaC$ and $PK_{CA}$, belong to the following language:
$\huaL_{T}:= \{ t_i,\alpha_\huaC,PK_{CA} \mid \exists (PK_i,cert_i,SK_i)$ s.t. $t_i= H(\alpha_\huaC,PK_i,cert_i,H(SK_i))\wedge pair(PK_i,SK_i)=1\wedge validate(PK_i,cert_i,PK_{CA})=1\}$, where the $validate$ function (as shown in Alg.\ref{contract1}) checks whether $PK_i$ is properly certified by CA. 

In this round, $t_i$ together with $\pi_i$ forms an actual anonymous credential. It will not only hide the identity of $W_i$, but also enable $\huaC$ to verify that the anonymous worker indeed owns an valid identity (although not revealed).
 %where $\vec{w} := (SK_W, cert)$ is secret witness of the owner of $cert$. Again, the zk-SNARK can be universally achieved through boolean circuit satisfiability. A boolean circuit $C_T(\vec{x},\vec{w})$ is constructed to represent the above constraint relationship of public knowledge and witness. The NP-complete language set therefore can be rewritten into $\bm{L}_{\bm{T}}:= \{\vec{x} \mid \exists \vec{w}$ s.t. $C_T(\vec{x},\vec{w})=0\}$.

\item {\em Round 3 \& 4}. Same as basic protocol.

\end{itemize}


\ignore{%%%%%%%%
1) \textbf{KeyGen}. CA generates a key pair $(PK_{CA},SK_{CA})$. The public key $PK_{CA}$ is sent to the blockchain such that it becomes public knowledge.

2) \textbf{WorkerKeyGen}. When requesting a certificate, a worker generates a key pair $(PK_{W},SK_{W})$. The worker sends CA the public key $PK_W$ and a blockchain address $W$.
%In this anonymous scheme, it doesn't matter that the worker owns $W$ or not.

3) \textbf{Sign}. After checking the identity of the worker, CA signs and issues a certificate $cert=(W, PK_W,\delta)$ to the worker, where $\delta:=sign(cert,SK_{CA})$ is CA's unforgeable signature.

4) \textbf{CredentialGen}. When the worker is participating in a task contract whose blockchain address is denoted by $C$, she generates an anonymous $token$ equal to $h(PK_W\|C)$ and a zk-SNARK proof $\pi$ for the correctness of $token$. The function $h(\cdot)$ is a collision-resistant hash function.

5) \textbf{CredentialVerify}. The contract performs a zk-SNARK verification by using public knowledge (i.e. $C$, $token$, $PK_{CA}$) and the zk-SNARK proof $\pi$. If and only if the verification passed, the contract confirms that the worker owns a valid certificate.
}%%%%%%%%

%In the above scheme, the zk-SNARK proof $\pi$ is attached to attest the statement that public knowledge $\vec{x} = (token,C,PK_{CA})$ belongs to the following NP-complete language set $\bm{L}_{\bm{T}}:= \{\vec{x} \mid \exists \vec{w}$ s.t. $ pair(SK_W,cert.PK_W)=1 $ $\wedge $ $token = h(PK_W\|C)$  $\wedge $ $vrfy( { cert, cert.\delta ,PK_{CA}} ) = 1 \}$, where $\vec{w} := (SK_W, cert)$ is secret witness of the owner of $cert$. Again, the zk-SNARK can be universally achieved through boolean circuit satisfiability. A boolean circuit $C_T(\vec{x},\vec{w})$ is constructed to represent the above constraint relationship of public knowledge and witness. The NP-complete language set therefore can be rewritten into $\bm{L}_{\bm{T}}:= \{\vec{x} \mid \exists \vec{w}$ s.t. $C_T(\vec{x},\vec{w})=0\}$.


\renewcommand{\algorithmicrequire}{\textbf{Input:}} % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm
\SetKwProg{Fn}{function}{}{}
\SetKwInOut{Require}{Require}
\begin{algorithm}\small
\label{contract:anonymous}
  \caption{Collect anonymous answers  (an example)}
  \Require{This contract's address $\alpha_\huaC$; The anonymous credential of requester $(t_R,\pi_R)$; the public key of CA $PK_{CA}$; zk-SNARK verification key regarding anonymous token, $VK_0$; number of requested answers, $n$; task deadline in unit of block $T_{\bm{A}}$.}
 % \KwOut{$\bm{A}^{\ast}$; $\bm{W}$; $\bm{T}$.}
 
  Answer ciphertexts, $\bm{A}^{\ast}\leftarrow\emptyset$\;
  Workers' anonymous credentials and receiving accounts, $\bm{W}\leftarrow(\emptyset,\emptyset)$\;
 
  \If {$getBalance(\alpha_\huaC) < \tau \vee \neg identify (t_R, \pi_R)$}
  {
 	        $refundRemainingBalance()$\;   
 	\textbf{exit}; \Comment{Budget not deposited or requester not identified.}
  }
 
  $timer_{\bm{A}}\leftarrow$ a timer expires after $T_{\bm{A}}$\;

  \While {$\bm{A}^{\ast}.length < n \wedge timer_{\bm{A}}$ NOT expired}
  {
    \If {$W_i$ sends $t_i,\pi_i,C_i,\alpha_i$}
    {
        \If {$\neg t_i = t_R \wedge \neg \bm{W}.contains(t_i) \wedge identify (t_i, \pi_i)$ }
        {
            {$\bm{W}.push(t_i, \alpha_i)$};
            {$\bm{A}^{\ast}.push(C_i)$};
        }
    }
  }
 % \textbf{return} $\bm{A}^{\ast}$, $\bm{W}$, $\bm{T}$\;

  \Fn{$identify (t,\pi)$}{
    $\vec{x} \leftarrow (t,\alpha_\huaC,PK_{CA})$\;
    \textbf{return} $libsnark.verifier(VK_0,\vec{x},\pi)$\;
  }
  \Fn {$refundRemainingBalance ()$}
{
	$transfer(\alpha_\huaC$, $\alpha$, $getBalance(\alpha_\huaC))$; \Comment{Refund balance}
}
%\vspace{-2mm}
\end{algorithm}


%
%In the scheme, instead of transparently submitting a certificate to a task contract, a worker sends an anonymous token. The token is generated from a valid certificate and the address of the task contract, by a collision-resistant hash function $h(PK_W\|addr)$, such that the token cannot be linked to either the certificate or another token that is generated by the same certificate but for a different contract. Along with the anonymous token,
\noindent \textbf{Same-prefix-linkable anonymous credential.} In the {\em Round 2}, we essentially construct a novel anonymous credential scheme having subtle linkability: the anonymous credentials of a worker can be linked, only when they are submitted to a same task (i.e. the worker produces them with a common-prefix). Although the concept can be instantiated through partially blind signature \cite{LC14}, our one-shot scheme is non-interactive and does not require the credential issuer (CA) to involve. 

More interestingly, the delicate linkability is a new concept different from either the classical linkable anonymous credential \cite{CL01} or the blacklistable anonymous credential \cite{TAK07}. The classical linkability of anonymous credential can prevent the anonymity misuse through linking all credentials generated by a user, while our delicate linkability can provide more fine-grained revocation of anonymity: if one misuses anonymity in a particular task, his anonymous credentials will be linkable in this single task only. The blacklistable anonymous credential requires workers to do a heavy proof attesting that their credentials are not in a public blacklist, and the proof will become heavier and heavier with the growth of the blacklist for all (honest) workers; in contrast, we observe the special requirement of a delicate linkability in crowdsourcing, and push the proving of anonymous credentials to be relatively light and constant (see Section \ref{implementation} for our experiment results).

In this paper, we just shed a light on the subtle property of our {\em same-prefix-linkable} anonymous credential and remark that it might be of independent interests. We remark that more detailed discussions about the scientific and use-cases behind are out scope of the paper.



\noindent \textbf{Correctness, efficiency and security.} Correctness and efficiency are similar to the basic protocol, except that each worker generates a zk-SNARK proof (instead of signing the ciphertext) to attest that he owes a public key certified by CA. Clearly, the smart contract can always identify an anonymous worker that follows the protocol, under that condition that the underlying SNARK is correct and the blockchain can be modeled as an ideal public ledger.
Moreover, the proof is for a correctly computed hash with inputs having message-signature pair structure and can be further optimized.

%Regarding security, let us first check anonymity.

Regarding the {\em worker anonymity}, let us consider a simplified security game, the adversary $\huaA$ has a token $t_0$ for $W_0$ in one task; now, in a different task, $\huaA$ receives one more token $t_b$ computed by hashing $(\alpha_\huaC,PK_b,cert_b,H(SK_b))$ together with a proof $\pi_b$ and a ciphertext $C_b$, from either $W_0$ or $W_1$, and will try to predict $b$. It is clear that both $\pi_b$ and $C_b$ leak nothing about $PK_b$, $SK_b$ or $cert_b$, because they can be simulated with public knowledge for the {\em zero-knowledge} of SNARK and the semantic security of the public key encryption, respectively. More importantly, $SK_b$ is unpredictable for $\huaA$, since the token value will be uniform to $\huaA$ when $H$ is a random oracle. So $t_b$ looks uniform to the adversary, even if it is conditioned on that she has an auxiliary $t_0$. This is clear because of the random oracle property of the hash function when inputs are not fully predictable.

\ignore{
Regarding {\em unlinkability between a worker and his answer}, if we use the security game to argue, it goes simply as follows. The adversary $\huaA$ receives a token $t_i$ computed by hashing $(\alpha_\huaC,PK_i,cert_i,H(SK_i))$, together with a proof $\pi_i$ and a ciphertext $C_i$. Both $\pi_i$ and $C_i$ leak nothing about $PK_i$, $SK_i$ or $cert_i$, because they can be simulated with public knowledge for the {\em zero-knowledge} of SNARK and the semantic security of the public key encryption, respectively. More importantly, $SK_i$ is unpredictable for $\huaA$, since the token value will be uniform to $\huaA$ when $H$ is a random oracle. We conclude that $\huaA$ cannot tell $t_0$ from $t_1$ for any two workers $W_0$ and $W_1$.

Regarding {\em unlinkability among all tasks of one worker}, let us consider a simplified security game (general definition can be argued similarly), the adversary $\huaA$ has a token $t_0$ for $W_0$ in one task; now $\huaA$ receives one more token $t_b'$ for a different task (together with the ciphertext and proof) from $W_0$ or $W_1$, and will try to predict $b$. Similar to the above unlinkability, $t_b'$ looks uniform to the adversary, even if it is conditioned on that she has an auxiliary $t_0$. This is clear because of the random oracle property of the hash function when inputs are not fully predictable. (The ciphertext and proof leak nothing about the token's inputs as they can be simulated as before.)
}

We also remark that the above anonymity is strong, since it holds even if the CA and the blockchain are corrupted. Therefore, we can propose the following formal theorem regarding to the worker anonymity.

\begin{theorem}
Conditioned on that the hash function to be modeled as a random oracle and the zk-SNARK doen by the worker is of zero-knowledge, our anonymous protocol satisfies the worker anonymity.
\end{theorem}

\ignore{%%%%%%%%%%%%%
	\begin{proof}
		We defer the formal proof to an extended version.
	\end{proof}
}%%%%%%%%%%%%%%%%%%%


Last, the other security properties are very similar to those in the previous basic protocol, except that workers send anonymous credentials attesting their identities (see Appendix A for the security of the anonymous credentials), and we can propose the following formal theorem for the anonymous protocol.
%We omit the details and the formal theorem similar to {\em Theorem \ref{thm:basic}} due to page limitation.


\begin{theorem}
Conditioned on that the blockchain we rely on can be modeled as an ideal public ledger, the hash function to be modeled as a random oracle, the underlying digital signature is secure, the public key encryption is semantically secure, and the zk-SNARK is both zero-knowledge and sound, our anonymous protocol satisfies: the worker anonymity, and all securities presented in our basic protocol.
\end{theorem}

\ignore{%%%%%%%%%%%%%
	\begin{proof}
		We defer the formal proof to an extended version.
	\end{proof}
}%%%%%%%%%%%%%%%%%%%



%The scheme has following important properties:

%$\bullet$ \emph{Unforgeability}.
%Loosely speaking, no matter what a prover is used, no proof can be produced to pass the zk-SNARK verification except some negligible probability when $C(\vec{x},\vec{w}) \neq 0$, which is know as the \emph{proof-of-knowledge} of zk-SNARK. Thanks to the \emph{proof-of-knowledge}, a proof for an anonymous token cannot pass the above zk-SNARK verification without a signed certificate and its paired secret key as witness, except some negligible probability. In addition, a worker owning one valid certificate can always generate one and only one token passing the above zk-SNARK verification in a given contract, which is a result of the \emph{completeness}, \emph{proof-of-knowledge} and the constraint $C_T(\vec{x},\vec{w})=0$. Therefore, if one cannot forge certificates, one cannot forge tokens.

%$\bullet$ \emph{Basic anonymity}. The proof $\pi$ is a zero-knowledge, and $token:=h(PK_W\|C)$ is generated by a one-way-like function $h(\cdot)$. Thus, an anonymous token cannot be linked to a worker's digital certificate, such that the privacy requirement P1 defined in Section II is achieved.

%$\bullet$ \emph{Unlinkability among contracts}. Recall that $h(\cdot)$ is a collision-resistant hash function and $token:=h(PK_W\|C)$. Therefore, valid tokens of a worker for different contracts cannot be linked, except some negligible probability.

%$\bullet$ \emph{In-contract linkability}. If one contract receives several valid tokens generated by one same certificate, they can be linked for sure by checking equality. This property can be understood as a consequence of the \emph{Unforgeability}.

%
%
%\begin{lemma}\emph{(Informal)}.
%Give validly signed certificate $cert=(W,PK,\sigma)$ and paired secret key $SK$ as only witness, $\exists token$ such that $(token,addr,PK_{CA})$ can pass the above zk-SNARK verification in the task contract $addr$.
%\end{lemma}
%\begin{proof}
%If $token=h(PK\|addr)$, a prover can use witness $(SK, cert)$ and public knowledge $(token,addr,PK_{CA})$ to construct a proof $\pi$ that can pass the verification, because zk-SNARK is of the completeness. Proved.
%\end{proof}
%
%
%\begin{lemma}\emph{(Informal)}.
%Give validly signed certificate $cert=(W,PK,\sigma)$ and paired secret key $SK$ as only witness, $\nexists token \neq h(PK\|addr)$ such that $(token,addr,PK_{CA})$ can pass the above zk-SNARK verification in the task contract $addr$ except some negligible probability.
%\end{lemma}
%
%\begin{proof}
%Prove by contraindication. Recall the \emph{proof-of-knowledge} of zk-SNARK. Assume there are two different $token$ and $token^\prime$. And $token$ and $token^\prime$ subject to that $(token,addr)$ and $(token^\prime,addr)$ can pass verification for sure, only if $token$ and $token^\prime$ are generated from two different public keys $PK$ and $PK^\prime$. There are two different $PK$ and $PK^\prime$, only if there two different certificates $(W,PK,\delta)$ and $(W,PK^\prime,\delta)$ as witness, respectively. Proved.
%\end{proof}
%
%
%
%\begin{theorem}\emph{(Informal)}.
%Give validly signed certificate $cert=(W,PK,\sigma)$ and paired secret key $SK$ as only witness, there exists a unique $token=h(PK\|addr)$ such that $(token,addr,PK_{CA})$ can pass the above zk-SNARK verification in the task contract $addr$ except some negligible probability.
%\end{theorem}
%
%\begin{proof}
%It is clearly true because of \emph{Lemma 3} and \emph{Lemma 4}.
%\end{proof}
%



\ignore{%%%%%%%%%%%old system

\section{SEPRIDE}\label{sec3-1}

Taking advantage of the mentioned schemes, we design a SEcure and PRIvacy-preserving DEcentralized data crowdsourcing system, SEPRIDE. The version 1.0 of SEPRIDE is promising to eliminate free-riding, false-reporting, data leakage and Sybil attack.  Furthermore, the version 2.0 of SEPRIDE is improved to respect the privacy of workers.

%SEPRIDE is based on two new schemes, i.e. leakage-free in-contract verification scheme and single-contract-linkable anonymous scheme. The former one is devised to allow contracts verify the quality of encrypted answers without decryption. The latter one is invited to enable contracts identify workers without linking their identity to them.


\subsection{SEPRIDE in a nutshell}\label{sec3-1}

As shown in Fig.5, the decentralized application (DApp) of SEPRIDE is made of an in-chain part and an off-chain part. The in-chain part consists of crowdsourcing task contracts and a callable interface of PKI DApp. The off-chain part consists of requester clients and worker clients. These clients are indeed blockchain clients (e.g. miner, full node or light-weight node) wrapped with some other functionalities. Requesters and workers do not have direct connections, and all transactions and communications are through task contracts posted by requesters. Active workers in the blockchain can review and verify details (e.g. the task description, the plan of rewarding, the public key, etc.) of a task contract. A worker can send her encrypted answer to the task contract if she decides to participate in the task. The encryption scheme used to protect answers from leakage is 2048-bit RSA-OAEP.

%A worker can join a task contract by submitting her answer encrypted by 2048-bit RSA-OAEP.

%Facing the transparency of smart contracts, SEPRIDE employs 2048-bit RSA-OAEP to protect data from leaking.

%It is arguable that data storage can be outsourced to some trusted data centers, such that contracts can just store digests. As a result, the encryption seems to be redundant. But we envision decentralism will more encourage decentralized off-chain storages. These off-chain storages \cite{Filecoin}\cite{ANS16} could be transparent as well. So SEPRIDE targets a scenario where all data storage is absolutely transparent.


\begin{figure}[!h]
\centering
\includegraphics[width=8cm]{fig3.eps}
\caption{The system-level view of SEPRIDE.}
\label{fig3}
\end{figure}


In SEPRIDE, a worker register through PKI to get her unique credential, a digital certificate. We notice the decentralization of PKI \cite{Alb17}\cite{ANS16} is a recent hotspot. However, PKI DApp as a public service is not immediately available at the time of writing, and the implementation of such decentralized PKI is out the scope of this paper. Alternatively, centralized PKI can be connected to blockchain-based oracle (information arbiters) to provide certifying service \cite{Swan15}. Although centralized PKI brings a risk of a central point of failure, it can be used in our proof-of-concept study where data crowdsourcing is urgently decentralized instead of PKI.

\ignore{%%%%%
\begin{figure}[!h]
\centering
\includegraphics[width=8cm]{fig5.eps}
\caption{Technical procedures of constructing the zk-SNARK in leak-free in-contract verification scheme.}
\label{fig2}
\end{figure}
}%%%%%%%

SEPRIDE heavily depends on zk-SNARKs to fight with the transparency of smart contracts. We use libsnark, an implementation of zk-SNARK for circuit satisfiability, to construct all zk-SNARKs required in SEPRIDE. Libsnark has proved \emph{completeness} and \emph{zero-knowledge}, and its \emph{soundness} and \emph{proof-of-knowledge} holds when the key generation phase is secure\footnotemark{}. A boolean circuit representing the relationship of public knowledge and secret witness is the fundamental step of constructing a zk-SNARK. We build up some gadgets (i.e small boolean circuits) including a gadget of 2048-bit modular exponentiation, a gadget of SHA-256 and some gadgets of quality estimation algorithms. Boolean circuits for the construction of zk-SNARKs are assembled by these small gadgets. Once the libsnark generator receives an assembled boolean circuit, it can produce a proving key $\sigma$ and a verification key $\tau$ for prover and verifier, respectively. The libsnark prover can use the proving key, public knowledge and secret witness to produce a NIZK proof for its statement. The libsnark verifier can verify the trueness of the statement, by the verification key, the proof and public knowledge. A pair of $\sigma$ and $\tau$ can be reused. For example, only one pair of $\sigma$ and $\tau$ is necessary in the single-contract-linkable anonymous credential scheme, since they can be repeatedly used by all provers (i.e. workers) and verifiers (i.e. contracts), respectively.

\footnotetext{
The key generation phase of libsnark might result in so-called ``toxic waste'' issue. The issue arises a worry of forged proofs, although no privacy can be violated. Multi-party computation is a promising way to securely generating libsnark keys. In this paper, we assume libsnark keys for a particular task have been securely generated.
}

Libsnark provers are incorporated into worker clients and requester clients. Requester clients need libsnark provers to construct NIZK proofs attesting the correctness of estimated qualities. Worker clients need libsnark provers to prove they own valid certificates. Libsnark verifiers are incorporated in the blockchain, such that zk-SNARK verifications in smart contracts can be executed and enforced by the blockchain community.
%Recently, an emerging crypto-currency, Zcash incorporates the libsnark verifier for a particular zk-SNARK, indicating the libsnark verifier is efficient enough to be deployed in the real-world blockchain.
%Additionally, a business-level libsnark verifier for general zk-SNARKs has been on the way to the real-world blockchain for a while.
Considering the fact that a business-level libsnark verifier is on the way to Ethereum, we fork\footnotemark{} Ethereum Virtual Machine by adding an operation code of libsnark verifier to prove the concept of SEPRIDE.
%Our fork\footnotemark{} of Ethereum can verify general zk-SNARKs including the ones used in our cryptographic schemes.

\footnotetext{The source code is available at https://github.com/Maxilbert/ethereumj}

\subsection{SEPRIDE v1.0}

In v1.0 of SEPRIDE, we consider the following design requirements to approach secure decentralization of data crowdsourcing: \emph{free-riding and false-reporting are discouraged; and meanwhile, answers are protected from leakage}. A prototype smart contract of v1.0 is briefly depicted in Algorithm 2 as pseudocode. To clarify the main idea behind, we assume that enough workers are interested in the contract.





\noindent \textbf{Analysis} Generally speaking, design requirements are realized by combining self-enforced smart contracts with the leakage-free in-contract verification scheme and the PKI scheme. The idea behind is as clear as: 1. data does not leak because 2048-bit RSA-OAEP is computationally secure and zk-SNARK is zero-knowledge; 2. the PKI scheme ensures no colluded answers submitted by Sybil attackers, such that the quality estimation algorithm seems effective; 3. the leakage-free in-contract verification scheme ensures that requesters are securely incentivized to be honest-reporters.

Honest-reporters are incentivized as following. After encrypted answers have been collected, the contract immediately starts an internal timer expiring in $T_{due}$ blocks. To get deposit refunded, the requester has to timely report qualities before timer expiring. The requester can agree that all answers are qualified, and the contract will automatically reward all workers. Alternatively, the requester can report detailed qualities of answers with a zk-SNARK proof. The leakage-free in-contract verification scheme is used to incentivize honest-reporting, because the scheme ensures that a false-reporter cannot get deposit refunded.


%In general, the prototype task includes the following sequential states:
%
%1) \textbf{Creating a task}. The requester has to send all necessary parameters (e.g. her public key, description of the task, the number of required answers, etc.) along with some security deposit. The deposit should include two parts: one part covers all possible rewards; the other part, called baseline deposit, can incentive the requester report qualities in time. The deposit will be enforced by the task contract.
%
%2) \textbf{Collecting answers}. A worker encrypts her answer with the public key of the requester. Besides the encrypted answer, the worker also submits her digital certificate through a blockchain transaction from her blockchain address, denoted $W$. The contract checks three points to verify the validity of the identity of the worker: 1. the certificate is validly signed by CA; 2. the blockchain address in the certificate is same to $W$; 3. the certificate has not been used in the task. If the above verification passing, the contract will collect the encrypted answer and record its associated $W$.
%
%3) \textbf{Honoring rewards}. After $M$ answers are collected, the requester is incentivized to timely report qualities of collected answers. If the requester does not prompt the contract of qualities in time, the baseline deposit will not be refunded to her as a penalty, and all answers will receive the promised reward. The requester can report qualities to the contract in two different ways. In the first option, the requester can agree that all answers are qualified, and the contract will automatically reward all workers. In the second option, the requester can report detailed qualities of answers with a zk-SNARK proof attesting that she is honestly reporting. \emph{Theorem 1} holds in SEPRIDE because RSA secret key is unique for the uniqueness of  modular multiplicative inverse. So the contract can always reveal the reported qualities are honest or not. As receiving honest-reporting, the contract will only transfer rewards to workers who submit qualified answers; otherwise, the contract will automatically reward all.

%\noindent \textbf{Analysis} The achievement of design requirements can be intuitively analyzed as following. Sybil attackers cannot get advantage if unforgeable certificates are issued by a trusted CA. As a result, the quality estimation algorithms seem to be effective with the honest majority assumption. It is worth to noticing that the quality of an answer can be more generally estimated by a different task although we do not consider this methodology in the above prototype. The prevention of data leakage is also straightforward, because all answers are encrypted by 2048-bit RSA-OAEP and zk-SNARK proofs are zero-knowledge. Detailedly, as long as the basic security assumption of RSA-OAEP holds, it seems computationally difficult to get advantage of answers' ciphertexts without the secure key; based on the zero-knowledge property of zk-SNARKs, the proof for qualities will ensure that no distinguisher can get non-negligible advantage of secret witness (i.e. secret key and unencrypted answers) as well. Free-riding is discouraged because our leakage-free in-contract verification scheme enables a requester convince the contract to pay free-riders nothing. The elimination of false-reporting is also owing to the scheme, because the contract can find any false-reporter and take an action to make the false-reporter get no advantage of the misbehavior.

\noindent \textbf{Extensions} Recall that the quality of each answer can be revealed and then be linked to the worker who submits it. A reputation-based incentive mechanism (e.g. reputation-based auction) is compatible with the version 1.0 of SEPRIDE to realize long-term fairness. %, although we apply quality-depended reward in the above prototype.
Such an extension might involve much trivial engineering work (e.g. the design of worker/requster profile contracts to keep track of reputations, the incorporation of reputation-based auction, etc.), and we will not discuss details in this proof-of-concept paper. %Besides, some other interesting extensions could be the incorporation of various auction mechanisms. Again, these extensions are mostly trivial engineering work and details will not be covered here.

\subsection{SEPRIDE v2.0 (anonymous mode)}

The v2.0 extends v1.0 in the aspect of respecting worker privacy. The v2.0 is compatible with v1.0 and can be seen as a plugin of SEPRIDE for privacy. We consider the privacy requirements P1 and P2 discussed in Section II, namely, \emph{the unlinkability between a worker and her tasks} and \emph{the unlinkability among tasks that a worker joins}.




Our single-contract-linkable anonymous credential scheme can be straightforwardly used in SEPRIDE to achieve these requirements. The scheme can be incorporated into the state of collecting answers by overloading the function of identifying workers, as illustrated in Algorithm 3.
%Two points are checked to identify a worker: 1. the token can pass the zk-SNARK verification of the anonymous credential scheme; 2. the token has not been used before in the task.


%The pseudocode of collecting anonymous answers in SEPRIDE v2.0 is illustrated in Algorithm 3. Except the part of identifying workers, the v2.0 prototype task is as same as the v1.0 prototype task.
%However, it is worth to noticing that a trivial reputation system cannot work in SEPRIDE v2.0 due to broken linkability. Although several anonymous reputation system are proposed, it is clear that they cannot work in SEPRIDE v2.0 because the idea behind them is still linkability. A system without the help of linkability will be our future work.


%It is clear that answers do not leak, as long as the factorization of 2048-bit RSA modulus cannot be performed. The prevention of Sybil attack can be discussed as following. The contract enforces workers to register at a certificate authority (CA) to get certificates. After CA verifies the identity of a worker (e.g. through cellphone number, IMEI number, etc.) as valid, it will issue a certificate containing a blockchain address owned by the worker. When the worker participates in a task, she sends her answers along with the certificate from the specified address in the certificate, such that the contract can verify her identity is valid. If the certificates scheme is unforgeable, no one can cheat the contract if she is not registered.
%
%The fairness in a SEPRIDE task can be discussed as following, with the basic assumption that most workers are honest.
%1) If a worker is a free-rider because she sends a poor answer:
%The requester is incentivized to prove the low-quality to the contract, because the low-quality answers are not rewarded. As a consequence, the free-rider cannot cheat of the reward.
%2) If a requester is false-reporter, and she tries to claim a high-quality answer as low-quality:
%The zk-SNARK verification will fail as indicated by Theorem 1, and the requester cannot get deposit refunded. If the requester is rational, she will not make a false report.



%The slightly differences between a contract having no claiming/biding phase and a contract having one are shown in Fig.4 as well. The requester can initialize a specified contract with her 2048-bit RSA public key along with detailed information about the task such as descriptions, the deadline, incentives, the number of required answers, and the maximum number of answers each worker can send. If the task contract has no claiming/bidding phase, the following states can be summarized as:
%
%\begin{figure}[!h]
%\centering
%\includegraphics[width=8.5cm]{fig4.eps}
%\caption{State machines of a task contract (a) having no claiming/bidding phase or (b) having claiming/bidding phase.}
%\label{fig4}
%\end{figure}
%
%Depositing -- The requester has to fund enough deposit. Minimum deposit is calculated by the largest possible bonus multiplied by a deposit rate larger than one.
%
%Collecting -- The contract starts to collect answers. Workers encrypt answers with the public key of the requester. An encrypted answer must be submitted with a valid certificate. In SEPRIDE v1.0, all certificates are transparently sent to the blockchain.
%
%Timed-out -- It is timed out, when the deadline of a task is due but there are not enough answers collected. On this situation, the requester will have to make a decision to continue the collection or stop the collection. The requester is incentivized to make such a decision for her deposit.
%
%Collected -- If enough answers have been collected, the task will reject any new answer. Collected answers is a tuple of answers i.e. $\left\langle A_j \right\rangle$. To complete the task, the requester can send qualities of answers i.e. $\left\langle Q_j \right\rangle$ and the solution's digest i.e. $digest=hash(solution; salt)$. Along with $\left\langle Q_j \right\rangle$ and $digest$, a zk-SNARK proof is sent to the contract for proving their correctness. Once the zk-SNARK proof is passed, the contract will automatically honor quality-based rewards to all answers. In case more answers are preferred, the requester can also choose to restart the collection instead of completing the task. To restart the collection, the requester has to fund more deposit with a higher deposit rate.
%
%Completed -- The task is completed after all rewards are automatically honored, the requester can get remaining balance refunded. The salted digest can be used for verifying the source of the solution in its remaining lifecycle.
%
%If a contract has a claiming/bidding state, a worker must send a deposit with her claim/bid. The deposit will be refunded when the worker doesn't win in the claiming/bidding or when the worker does send answer(s) to the contract.
%
%Contract states are driven by external transactions (e.g. funds, a certificate, a zk-proof) or internal events (e.g. a timer of block number or a timer of block timestamp). Internal events are always trusted, because they are automatically generated by the blockchain. However, misbehavior might happen when external transactions are required to drive a contract. For example, a misbehaved worker can send an invalid certificate, while a misbehaved requester can send an invalid zk-SNARK proof. Once a SEPRIDE task contract finds a misbehavior, an exception will incur and contracts will handle with it. Besides some trivial exceptions (e.g. an arbitrary node instead of the requester sends a proof in the collected state), SEPRIDE can check and handle with the following main exceptions:
%
%E1. when collecting answers, if an answer is sent with an invalid certificate, the contract will simply drop it and continue to collection;
%
%E2. in the collecting state, if an answer is sent with a certificate whose owner has sent as many times as the contract allows, the contract will simply drop it and continue to collection;
%
%E3. when a contract stay in the collected state, if the requester sends a proof that fails in the zk-SNARK verification, the contract will confiscate the deposit of the requester and equally divide all remaining balance to each answer.
%
%The above processes of exception handling in SEPRIDE make rational workers and rational requesters have no interest in misbehavior (i.e. invalid certificate, duplicated certificate, invalid zk-SNARK proof).
%
%It is clear that threats T1 and T5 is easily solved after the introduce of smart contract, because a task contract can be trusted to temporarily hold deposits. Threat T2 and T3 are also solved by the asymmetric encryption and its important derivative -- certificate scheme, respectively. To solve T4, a contract has to be able to verify data quality; similarly, to solve T6, there must be a way for a contract to verify and store the digest of a solution. These issues become nontrivial, because any decryption in contracts will lead up to data leakage. A scheme based on zero-knowledge proofs is used to solve them.
%
%
%As illustrated in Fig.5, the zk-SNARK verifier is incorporated in the blockchain. The primary (public) inputs, the proof and the verification key are all accessible by a task contract, such that the zk-SNARK verification can be automatically enforced. What's more, zk-SNARK can guarantee auxiliary inputs are not leaked through the proof. So the private key of the requester, as an auxiliary input, is a secret of the requester, and no one can get extra advantage from the verification processes to attack the access control mechanism.
%
%It is clear that the contract can verify data qualities and the salted digest of the solution, as along as the verification result is ``PASS''. But one major concern is: ``will these verifications be efficient enough?'', since we know time-consuming operations in contracts might arise considerable security threat. The short answer is ``yes, it is efficient'', and we will show detailed evaluations in Section 5 later to demonstrate how feasible the scheme is.


\noindent \textbf{Analysis}
Thanks to the properties of our single-contract-linkable anonymous credential scheme, v2.0 prevents Sybil attack as well as guarantees remarkable unlinkability such as P1 and P2 in the DApp layer. Careless use of v2.0 might cause linkability in the blockchain layer, making all efforts in ruin. A way to the anonymity in blockchain layer is that worker clients use one-time addresses for all tasks, and a mixer contract (i.e. tumbler) is cooperatively used by a number of workers to anonymously merge rewards. The solution is immediate available in Ethereum where a ring signature mixer contract has been demonstrated a recent release. Besides mixers, other solutions could be available, but detailed discussion of them is outside the scope of this work.
}%%%%%%%%%

%%%%%%%%%old system




%
%\footnotetext{
%See https://blog.ethereum.org/2016/03/05/serenity-poc2/ for the implementation of ring signature mixer.}

%It is clear that design requirements such as P1 and P2 are achieved because of the mentioned properties of single-contract-linkable anonymous credential scheme. The prevention of Sybil attackers can be explained as following. There could be two kinds of successful Sybil attackers. First kind of attackers own no certificate but can generate valid tokens that pass the zk-SNARK verification, which is impossible as long as certificates cannot be forged. Second kind of attackers have some certificates and generate two or more valid tokens from one certificate, which is impossible because of \emph{Theorem 2}.

%A trivial reputation system cannot work in SEPRIDE v2.0 due to the broken linkability. What's worse, state-of-the-art anonymous reputation systems will not work in SEPRIDE v2.0, because the idea behind them is still linkability among tasks. How to keep track of reputations without linking is still an interesting open question. We will see a chance of solving this nontrivial issue in our future work.

%Although SEPRIDE v2.0 guarantees remarkable unlinkability in the DApp layer, careless use of SEPRIDE v2.0 will cause linkability in the blockchain layer, making all efforts on preserving privacy in ruin. For example, if a worker participates in all her tasks with only one blockchain address, her tasks will be linked through this blockchain addresses. In the following, we briefly point out a couple of possible ways to the unlinkability in the blockchain layer.

%1) Worker clients use one-time addresses for all tasks (or randomly use one out of many addresses). After receiving rewards, worker clients can join a mixing-service (i.e. tumbler) to merge rewards. The solution is straightforward and immediate available in Ethereum where a proof-of-concept ring signature mixer has been demonstrated since its Serenity PoC2 release\footnotemark{}.
%
%\footnotetext{
%See https://blog.ethereum.org/2016/03/05/serenity-poc2/ for the implementation of ring signature mixer.}



%2) A blockchain integrates both smart contract and anonymous transaction can be the final solution. Currently, although most smart contract enabled blockchains (e.g. Ethereum, HyperLedger) currently do not support anonymous transactions and most anonymous transaction enabled blockchains (e.g. Monero, Zcash) do not support smart contracts, Zcash is on the way to being integrated on Ethereum\footnotemark{}. The idea behind is a zk-SNARK verifier enabled Ethereum can realize anonymous transactions by the way used in Zcash \cite{SCG14}.
%
%\footnotetext{
%See https://z.cash/blog/zcash-eth.html for the integration of Zcash on Ethereum.
%}





